TeCH: Text-guided Reconstruction of Lifelike Clothed Humans

Despite recent research advancements in reconstructing clothed humans from a single image, accurately restoring the "unseen regions" with high-level details remains an unsolved challenge that lacks attention. Existing methods often generate overly smooth back-side surfaces with a blurry texture. But how to effectively capture all visual attributes of an individual from a single image, which are sufficient to reconstruct unseen areas (e.g., the back view)? Motivated by the power of foundation models, TeCH reconstructs the 3D human by leveraging 1) descriptive text prompts (e.g., garments, colors, hairstyles) which are automatically generated via a garment parsing model and Visual Question Answering (VQA), 2) a personalized fine-tuned Text-to-Image diffusion model (T2I) which learns the "indescribable" appearance. To represent high-resolution 3D clothed humans at an affordable cost, we propose a hybrid 3D representation based on DMTet, which consists of an explicit body shape grid and an implicit distance field. Guided by the descriptive prompts + personalized T2I diffusion model, the geometry and texture of the 3D humans are optimized through multi-view Score Distillation Sampling (SDS) and reconstruction losses based on the original observation. TeCH produces high-fidelity 3D clothed humans with consistent & delicate texture, and detailed full-body geometry. Quantitative and qualitative experiments demonstrate that TeCH outperforms the state-of-the-art methods in terms of reconstruction accuracy and rendering quality. The code will be publicly available for research purposes at https://huangyangyi.github.io/TeCH

==> figtex/qualitative-dataset-small.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[width=\linewidth]{fig/qualitative_dataset_small_1_compress.pdf}  
% \vspace{-2.0 em}
\caption{Zoom-in visualization of results of CAPE dataset and \thtwo dataset. \mn can reconstruct plausible clothed body shapes in callenging body poses. It also generates realistic 3D geometric details and high-quality textures with consistent color in back-side areas.} 
\label{fig:qualitative-dataset-small}
% \vspace*{-1. em} 
\end{figure*} 

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> paper/03_Method_bak.tex <==
 \section{Method} \label{sec:method} 
%
Given a single RGB image as input, \mn aim at reconstructing a high-fidelity 3D clothed human.
% 
Specifically, ``high-fidelity'' here refers to the inclusion of complete and consistent texture, as well as intricate geometric details. 
% 
To achieve this, \mn follow a two-step procedure:  
%
Firstly, text prompt to depict the input image is obtained via human parsing model SegFormer~\cite{xie2021segformer} plus VQA model BLIP~\cite{li2022blip} (\sref{sec:text_guidance}).
%
This descriptive prompt will guide the generation process in \db~\cite{ruiz2022dreambooth}, a personalized Text-to-Image diffusion model fine-tuned on augmented input images.
%
Secondly, the 3D human, which is represented as hybrid \dmtet and initialized from \smplx (\sref{sec:representation}), will be optimized (\sref{sec:optimization}) with SDS loss computed from the \db.
%
To enhance its geometric details and texture consistency, we employ a multi-stage optimization strategy (\sref{sec:multistage}).
%
%In the following, we first introduce a few preliminaries (\sref{sec:preliminaries}): \db, Score Distillation Sampling (SDS), \dmt, before delving into the specifics of our methodology in the subsequent sections.
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\yangyi{Are we removing this preliminaries section?}
\begin{comment}
\subsection{Preliminaries} \label{sec:preliminaries}

\qheading{DreamBooth}
%
Text-to-Image diffusion models trained on extensive text-image pair datasets (\eg \laion~\cite{schuhmann2022laionb}) can generate diverse and realistic images from a description in natural language, such as \sd~\cite{rombach2022high}, \imagen~\cite{saharia2022photorealistic}, and \dalle~\cite{rameshZeroShotTexttoImageGeneration2021,ramesh2022hierarchical}.
%
However, it is challenging to accurately describe the appearance of an ``unseen'' subject (\ie a subject that seldom appears in the training data) with text prompts to generate subject-specific images.
%
To enable subject-driven image generation, DreamBooth~\cite{ruiz2022dreambooth} presents a method for ``personalizing'' the diffusion model through few-shot tuning.
%

%
Specifically, for a pre-trained image diffusion model $\hat{\mathbf{x}}_\phi$, the model takes an initial noise $\epsilon\sim\mathcal{N}(0,1)$, and a text embedding $\mathbf{c}=\Gamma(P)$, generated by the text encoder $\Gamma$ and a text prompt $P$, to produce an image $\mathbf{x}_{\mathrm{gen}}=\hat{\mathbf{x}}_\phi(\epsilon, \mathbf{c})$.
%
The vanilla DreamBooth uses a small dataset comprising 3-5 images of the same subject to fine-tune the diffusion model using MSE denoising losses:
%
\begin{multline}
\mathbb{E}_{\mathbf{x},\mathbf{c},\mathbf{\epsilon},\mathbf{\epsilon'},t}  = \bigl[w_t\left\Vert\hat{\mathbf{x}}_\phi(\alpha_t\mathbf{x}_\mathrm{gt}+\sigma_t\mathbf{\epsilon}, \mathbf{c}) - \mathbf{x}_\mathrm{gt}\right\Vert_2^2 \\ + \lambda w_{t'} \left\Vert \hat{\mathbf{x}}_\phi(\alpha_{t'}\mathbf{x}_\mathrm{prior}+\sigma_{t'}\mathbf{\epsilon}', \mathbf{c}_\mathrm{prior})-\mathbf{x}_\mathrm{prior}\right\Vert_2^2\bigr]
\end{multline}
%
In the first term, $\mathbf{x}_\mathrm{gt}$ represents ground-truth images, and $\mathbf{c}$ is the embedding of a text prompt with a rare token as the subject unique identifier, while $\alpha_t$, $\sigma_t$, $w_t$ are terms controlling the noise schedule and sample quality of the diffusion process at time $t\sim\mathcal{U}([0,1])$.
%
The second term is the prior-preservation loss weighted by $\lambda$, which is supervised by self-generated images $\mathbf{x}_\mathrm{prior}$ conditioned with the class-specific embedding $\mathbf{c}_\mathrm{prior}=\Gamma(\text{``a man/woman''})$.
%
The prior-preservation loss is designed to prevent language drift and enhance output diversity.
%

\qheading{Score Distillation Sampling (SDS)}
%
\df~\cite{poole2022dreamfusion} introduces Score Distillation Sampling (SDS) loss, to perform Text-to-3D synthesis by using pretrained 2D Text-to-Image diffusion model $\phi$.
%
Instead of sampling in pixel space, SDS optimizes over the 3D volume, which is parameterized with $\theta$, with the differential renderer $g$, so the generated image $\mathbf{x}=g(\theta)$ closely resembles a sample from the frozen diffusion model.
%
Here is the gradient of $\mathcal{L}_\mathrm{SDS}$:
%
\begin{multline}
\nabla_\theta\mathcal{L}_\mathrm{SDS}(\phi, \mathbf{x}=g(\theta)) \\ = \mathbb{E}_{\mathrm{t, \epsilon}}\left[ w_t \left(\hat{\epsilon}_\phi(\mathbf{z}_t^\mathbf{x};\mathbf{c},t)-\epsilon\right)\frac{\partial \mathbf{x}}{\partial \theta}\frac{\partial \mathbf{z}^\mathbf{x}}{\partial \mathbf{x}}\right]
\end{multline}
%
where $\hat{\epsilon}_\phi(\textbf{z}_t^\mathbf{x}; \mathbf{c}, t)$ denotes the noise prediction of the diffusion model with condition $\mathbf{c}$ and latent $\mathbf{z}_t^\mathbf{x}$ of the generated image $\mathbf{x}$.
%
Such SDS-guided optimization is performed with random camera poses to improve the multi-view consistency. In contrast to \df, the 3D shape here is parameterized with improved \dmtet instead of NeRF. 
%

\qheading{Deep Marching Tetrahedra (\dmtet)}
\label{dmtet}
\dmtet~\cite{shen2021deep, gao2020learning} is a hybrid 3D representation designed for high-resolution 3D shape synthesis and reconstruction.
%
It incorporates the advantages of both explicit and implicit representations, by learning Signed Distance Field (SDF) values on the vertices of a deformable tetrahedral grid.
%
For a given \dmtet, represented as $(V_T, T)$, where $V_T$ are the vertices in the tetrahedral grid $T$, which comprising $K$ tetrahedrons $T_k \in T$, with $k \in \{1,\dots,K\}$, and each tetrahedron is defined by four vertices $\{v_{k}^1,v_{k}^2,v_{k}^3,v_{k}^4\}$. The objective of the model is firstly to estimate the SDF value $s(v_i)$ for each vertex, then to iteratively refine the surface and subdivide the tetrahedral grid by predicting the position offsets $\Delta v_i$ and SDF residual values $\Delta s(v_i)$.
%
This SDF is then converted into an explicit triangular mesh through Marching Tetrahedra~\cite{doi1991efficient}.
%
Magic3D~\cite{lin2022magic3d} highlights two strengths of \dmtet over NeRF: fast-optimization and high-resolution. It achieves this by efficiently rasterizing a triangular mesh into high-resolution image patches using a differentiable renderer~\cite{Laine2020diffrast}, enabling interaction with high-resolution latent diffusion models like \sd.
%
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Extracting Text-guidance from the Observation} 
\label{sec:text_guidance}

\mheading{Parsing human attributes from 2D image}
% 
Given the input human image, \segf\footnote{\url{https://huggingface.co/matei-dorian/segformer-b5-finetuned-human-parsing}}~\cite{xie2021segformer}, which is fine-tuned on ATR dataset~\cite{liang2015deep,liang2015human}, is firstly applied to recognize each part of the garments (\eg hat, skirt, pants, belt, shoes).
%
To obtain more precise and detailed descriptions (\ie color, style) of the parsed garments, we utilize the vision-language model BLIP~\cite{li2022blip} as VQA captioner. This model has been pre-trained on a vast collection of image-text pairs, enabling it to automatically generate descriptive prompts.

%
Rather than using naive image captioning, we employ a series of fine-grained VQA questions $\{Q_i\}$ (see details in \supmat) to inquire about BLIP. These questions cover garment styles, colors, facial features, and hairstyles, with the corresponding answers denoted as $\{A_i\}$.
%
The set of $\{A_i\}$ will be inserted into a predetermined template to create text prompts $P_\mathrm{VQA}$, which will serve as text-guidance to condition the text-to-image diffusion model.
%

\mheading{Embedding subject-specific with DreamBooth}
% 
Does the text prompt $P_\mathrm{VQA}$ comprehensively capture all the visual characteristics of the subject? No, a picture is worth a thousand words.
%
Thus, we also utilize \db~\cite{ruiz2022dreambooth} to learn the \textit{indescribable} visual appearance from the input image.
%
To prevent overfitting on \db, we augment each input image with five different backgrounds.
% 
To enhance the facial details, we employ a super-resolution model GFPGAN~\cite{wang2021gfpgan} to augment the face region.
%
To prevent language drift, we assign the subject classes in \db as ``man'' or ``woman'' based on the gender of the character.
%
After fine-tuning, the subject-specific appearance details are encoded within a unique identifier ``$[V]$'' in personalized \db $\mathcal{D}'$. 
%

%
Finally, we insert the identifier ``$[V]$'' into $P_\mathrm{VQA}$, to construct the final text prompt used by $\mathcal{D}'$, denote as $P$.
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Hybrid 3D Representation}% for High Resolution Textured Clothed Human}
\label{sec:representation}
%
To efficiently represent the 3D clothed human using a high-resolution mesh, we extend the \dmtet \cite{gao2020learning, shen2021deep} with a tetrahedral outer shell~\cite{Onizuka2020} around the \smplx body model. 
This involves constructing a more compact tetrahedral grid $(V_\mathrm{shell}, T_\mathrm{shell})$ within an outer shell $\mathcal{M}_\mathrm{shell}$, see~\cref{fig:method}-(c). The creation of $\mathcal{M}_\mathrm{shell}$ is achieved through a series of steps including mesh dilation, down-sampling, and up-sampling \wrt the body mesh $\mathcal{M}_\mathrm{body}$, which is parameterized using \smplx~\cite{pavlakos2019expressive} and estimated from the input image by \pixie~\cite{feng2021pixie}.

%
We use two MLP networks $\Psi_\mathrm{g}$ and $\Psi_\mathrm{c}$ with hash encoding~\cite{muller2022instant} to learn the geometry and color separately.
%
The geometry network $\Psi_\mathrm{g}$ locates the mesh surface implicitly by predicting \dmtet vertex SDF value, $s(v_i)$
\begin{equation}
    s(v_i; \psi_\mathrm{g}) = \Psi_\mathrm{g}(v_i)
\end{equation}
Here, $\psi_\mathrm{g}$ represents the parameters of $\Psi_\mathrm{g}$, which are initialized using $\mathcal{M}_\mathrm{body}$. To achieve this initialization, we employ the loss function $\mathcal{L}_\mathrm{init}$ to fit $\Psi_\mathrm{g}$ onto the SDF of $\mathcal{M}_\mathrm{body}$
\begin{equation}
    \mathcal{L}_\mathrm{init}=\sum_{p_i\in \mathbf{P}_\mathrm{}}\norm{s(p_i; \psi_\mathrm{g}), \mathrm{SDF}(p_i)}_2^2
\end{equation}
where $\mathbf{P}=\{p_i\in\mathbb{R}^3\}$ is a point set randomly sampled near $\mathcal{M}_\mathrm{body}$, and $\mathrm{SDF}(p_i)$ is pre-computed per-point SDF.
%
Triangular meshes can be extracted from this efficient hybrid 3D representation by Marching Tetrahedra (MT)~\cite{doi1991efficient}
%
\begin{equation}
\mathcal{M}(\psi_\mathrm{g})=\mathrm{MT}(V_\mathrm{shell} + \Delta V_\mathrm{shell}, T_\mathrm{shell}, s(V_\mathrm{shell})) 
\end{equation} 
%

In our \dmtet subdivision, a more detailed surface $\mathcal{M}_\mathrm{subdiv}(\psi_\mathrm{g})$ can be obtained by applying volume subdivision on the surface tetrahedra grids $(V_\mathrm{surface}, T_\mathrm{surface})$ that intersect with $\mathcal{M}(\psi_\mathrm{g})$, while the SDF values of the refined \dmtet vertices are also modeled by $\Psi_\mathrm{g}$.
%

%
Given camera $\mathbf{k}$, the generated mesh is rendered through differentiable rasterizer $\mathcal{R}$~\cite{Laine2020diffrast}, to get the back-projected 3D locations $\mathcal{P}(\psi_\mathrm{g}, \mathbf{k})$, rendered mask $\mathcal{M}(\psi_\mathrm{g}, \mathbf{k})$, and rendered normal map $\mathcal{N}(\psi_\mathrm{g}, \mathbf{k})$
%
\begin{equation}
    \mathcal{R}(\mathcal{M}(\psi_\mathrm{g}), \mathbf{k}) = \left(\mathcal{P}(\psi_\mathrm{g}, \mathbf{k}), \mathcal{M}(\psi_\mathrm{g}, \mathbf{k}), \mathcal{N}(\psi_\mathrm{g}, \mathbf{k})\right)
\end{equation}
% where $\mathbf{P}(\psi_\mathrm{g}, \mathbf{k})$ is the back-projected 3D locations of each rasterized pixels, $m(\psi_\mathrm{g}, \mathbf{k})$ is the differentiable mask of rasterization and $\mathcal{N}(\psi_\mathrm{g}, \mathbf{k})$ is the rendered normal map of the mesh under ca`mera $\mathbf{k}$. 
% 
The albedo of each back-projected pixel is predicted by color network $\Psi_\mathbf{c}$, where $\psi_\mathrm{c}$ represents the parameters
%
\begin{equation}
    \mathrm{Albedo}(\psi_\mathrm{g}, \psi_\mathrm{c}, \mathbf{k}) = \Psi_\mathbf{c}(\psi_\mathrm{c}, \mathcal{P}(\psi_\mathrm{g}, \mathbf{k}))
\end{equation}
% %
% We employ Lambertian shading in our rendering process, utilizing a light direction $l$ to generate 2D images that capture both texture and geometry details.
% %
% \begin{multline}
%     \mathcal{C}_\mathrm{shaded}(\psi_\mathrm{g}, \psi_\mathrm{c}, \mathbf{k},l) \\ = \mathrm{Albedo}(\psi_\mathrm{g}, \psi_\mathrm{c}, \mathbf{k})(\ell_p \mathcal{N}(\Psi_g, \mathbf{k})\cdot l + \ell_a)
% \end{multline}
% %
% where $\ell_p$ is the directional light strength, $\ell_a$ is the ambient light strength, and $\mathcal{C}_\mathrm{shaded}$ is the final color.
% %

% With the rasterized normal map $\mathcal{N(\psi_\mathrm{g}, \mathbf{k})}$ and the rasterized albedo map $\mathcal{C}(\psi_\mathrm{g}, \psi_\mathrm{c}, \mathbf{k})$, we can produce Lambertian shaded rendering with a light direction $l$, which reflects both texture and geometry details and is important for our joint optimization process explained in the next section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Decoupled Optimization of Geometry and Texture}
\label{sec:optimization}

\yangyi{We will merge Sec.3.4 and Sec.3.5 into a single section of decoupled optimization, maybe we can discuss losses for geometry and losses for texture seperately.}

\subsubsection{Geometry-stage}
\mheading{Pixel-aligned silhouette loss}

\qheading{SDS loss on normal images}

\qheading{Geometric regularization with normal estimation}

\qheading{Overall losses}

\subsubsection{Texture-stage}

\qheading{Pixel-aligned reconstruction loss}

\qheading{SDS loss on color images}

\qheading{Chamfer-based color consistency loss}

\qheading{Overall losses}

\subsubsection{Camera sampling during optimization}
\yangyi{below are the original content of Sec. 3.4}

%
To optimize both the geometry network $\psi_{g}$ and the texture network $\psi_{c}$ simultaneously, we employ pixel-wise reconstruction loss, score distillation sampling (SDS) loss, and geometry regularization loss.
%

\qheading{Pixel-wise reconstruction loss} 
%
In each optimization step, we employ an image reconstruction loss to enforce input-view consistency, which is applied between input image $\mathcal{I}$ and albedo-rendered image.
%
\begin{align}
\begin{split}
    \mathcal{L}_\mathrm{recon} &= \lambda_\mathrm{MSE} \norm{\mathcal{I}, \mathrm{Albedo}(\psi_\mathrm{g}, \psi_\mathrm{c}, \mathbf{k_\mathcal{I}})}_2^2 \\ &+ \mathrm{LPIPS}(\mathcal{I}, \mathrm{Albedo}(\psi_\mathrm{g}, \psi_\mathrm{c}, \mathbf{k_\mathcal{I}}))
    \label{recon-loss}
\end{split}
\end{align}
%
where $k_\mathcal{I}$ denotes the input view camera, and $\lambda_\mathrm{MSE}$ is a weight to balance the two loss term. 
%
To produce pixel-aligned geometry, a silhouette loss~\cite{zhangPerceiving3DHumanObject2020, yiHumanAwareObjectPlacement2022} is introduced:
%
\begin{align}
\begin{split}
    \mathcal{L}_\mathrm{mask} &= \norm{\mathcal{S}, \mathcal{M}(\psi_\mathrm{g}, \mathbf{k})}_2^2 \\ &+ \sum_{x\in \text{Edge}(\mathcal{M(\psi_\mathrm{g}, \mathbf{k})})}\min_{\hat x\in \text{Edge}(\mathcal{S})}\norm{x-\hat{x}}_1 ,
\end{split}
\end{align}
%
which consists of 1) a pixel-wise L2 loss over the foreground mask $\mathcal{S}$ and the rendered silhouette $\mathcal{M}$, 2) edge distance loss, based on the distance of each silhouette boundary pixel $x\in\text{Edge}(\mathcal{M}(\psi_\mathrm{g}, \mathbf{k}))$ to the nearest foreground mask boundary pixel $\hat{x}\in\text{Edge}(\mathcal{S})$

\qheading{SDS loss on both normal and color images}
%
To recover the full-body geometry, including unseen regions, while ensuring view-consistent texture, we employ a joint update on $\{\psi_\mathrm{g},\psi_\mathrm{c}\}$ via SDS loss $\mathcal{L}_\mathrm{SDS}^\mathrm{c}$. This loss is calculated based on random-view color renderings $\mathbf{x}=\mathrm{Albedo}(\psi_\mathrm{g}, \psi_\mathrm{c}, \mathbf{k})$, and the \db $\mathcal{D}'$ guided by text prompt $P$.
%
\begin{multline}
    \nabla_{\{\psi_\mathrm{g}, \psi_\mathrm{c}\}}\mathcal{L}_\mathrm{SDS}^\mathrm{color}(\mathbf{x}, \mathbf{c}^P) \\
    = \mathbb{E}_{\mathrm{t, \epsilon}}\left[ w_t \left(\hat{\epsilon}_{\phi'}(\mathbf{z}_t^\mathbf{x};\mathbf{c}^P,t)-\epsilon\right)\frac{\partial \mathbf{x}}{\partial \{\psi_\mathrm{g}, \psi_\mathrm{c}\}}\frac{\partial \mathbf{z}^\mathbf{x}}{\mathbf{x}}\right], 
    \label{sds-color-loss}
\end{multline} 
%
where $\mathbf{k}$ is the camera pose, $\mathbf{c}^P$ is the text embedding of $P$, $\phi'$ is the parameter of $\mathcal{D}'$.
% , and $\mathcal{L}_\mathrm{SDS}^\mathrm{color}$ is weighted by $\lambda_\mathrm{SDS}^\mathrm{color}$.
%

%
However, since the geometry and texture are highly entangled in the rendering, relying solely on supervision from the rendered RGB image can potentially yield degenerated results, such as noisy or excessively smoothed geometry.
%
To address this issue, inspired by \fd~\cite{chen2023fantasia3d}, our approach integrates normal renderings alongside color renderings. This incorporation enables \mn to effectively capture intricate geometric details.
% 
Specifically, we generate the surface normal maps, denoted as $\mathbf{n}=\mathcal{N}(\psi_\mathrm{g}, \mathbf{k})$. These maps are utilized similarly to the albedo image $\mathbf{x}$ for computing the SDS loss and updating the parameter $\psi_\mathrm{g}$.
%
\begin{multline}            \nabla_{\psi_\mathrm{g}}\mathcal{L}_\mathrm{SDS}^\mathrm{normal}(\mathbf{n}, \mathbf{c}^{P_\mathrm{normal}}) \\
= \mathbb{E}_{\mathrm{t, \epsilon}}\left[ w_t \left(\hat{\epsilon}_{\phi'}(\mathbf{z}_t^\mathbf{n};\mathbf{c}^{P_\mathrm{normal}},t)-\epsilon\right)\frac{\partial \mathbf{n}}{\partial \psi_\mathrm{g}}\frac{\partial \mathbf{z}^\mathbf{n}}{\mathbf{n}}\right], 
\end{multline}
%
where $\mathbf{c}^{P_\mathrm{normal}}$ is the text condition with an augmented prompt $P_\mathrm{normal}$. 
% 
We construct $P_\mathrm{normal}$ from $P$ by adding an extra description "a detailed sculpture of" to better reflect the intrinsic characteristics of normal maps.
%

%
Moreover, to enhance the coherence of geometric and textural details during the joint optimization procedure. Same as \df~\cite{poole2022dreamfusion}, we introduce an additional supervision loss through applying the SDS loss on the shaded rendering, denoted as $\mathcal{L}_\mathrm{SDS}^\mathrm{shaded}$. The formulation of $\mathcal{L}_\mathrm{SDS}^\mathrm{shaded}$ is identical to that of $\mathcal{L}_\mathrm{SDS}^\mathrm{color}$, see~\cref{sds-color-loss}; however, it incorporates an input image $\mathbf{x}_\mathrm{s}=\mathcal{C}_\mathrm{shaded}(\psi_\mathrm{g}, \psi_\mathrm{c}, \mathbf{k}, l)$ generated from a uniformly random light direction $l$.
%

\qheading{Geometric regularization with normal estimation}
%
We discovered that relying solely on reconstruction losses and SDS losses may lead to the generation of noisy surfaces that do not align well with the input image. This is particularly evident for subjects wearing complex clothing.
% 
To address this issue, we leverage the front \& back normal estimations as an additional constraint to regularize the reconstructed geometric surface:
%
\begin{multline}
    \mathcal{L}_\mathrm{norm}(\hat{\mathcal{N}}_\mathbf{k}, \mathbf{n}) \\ = \lambda_\mathrm{MSE_{norm}} \norm{(\hat{\mathcal{N}}_\mathbf{k}, \textbf{n})}_2^2 + \mathrm{LPIPS}(\hat{\mathcal{N}}_\mathbf{k}, \textbf{n})) ,
    \label{loss-normal}
\end{multline}
%
where $\hat{\mathcal{N}}_\mathbf{k}$ are the front \& back normal maps \textit{estimated} from the input image by ICON~\cite{xiu2022icon}, $\mathbf{k}$ is the camera pose, $\mathbf{k} \in \{\mathrm{front}, \mathrm{back}\}$. And $\mathbf{n}$ is the normal maps \textit{rendered} from 3D shape $\Psi_\mathrm{g}$ under camera $\mathbf{k}$.
%
Same as the reconstruction loss in~\cref{recon-loss}, we use a combination of LPIPS and MSE loss to enhance the perceptual similarity between 
 $\hat{\mathcal{N}}_\mathbf{k}$ and $\mathbf{n}$. 
%
Furthermore, we utilize a regularization loss based on Laplacian smoothing~\cite{ando2006learning}, represented as $\mathcal{L}_\mathrm{lap}$, to effectively reduce the presence of noisy artifacts.
%

% \qheading{Concatenating reference image in SDS}
% %
% Inspired by the trick of concatenating multiple frames as the input of the diffusion model to generate consistent multi-frame rendering\cite{xanthius2023multiframe}, we propose an enhancement to the SDS loss on color images. With a chance of $p_\mathrm{concat}$, we concatenate the input image $\mathcal{I}$ to the color rendering $x$ after cropping as the input of $\mathcal{L}_\mathrm{SDS}^c$. This further encourages the generated views to have consistent clothing styles and colors with the input image.

\qheading{Chamfer-based color consistency loss} As previously mentioned in \df~\cite{poole2022dreamfusion}, the SDS loss may result in over-saturated color. For our method, this will cause a noticeable color disparity between visible and invisible regions. To mitigate this issue, we incorporate a color consistency loss to ensure that the rendered novel views align closely with the color distributions observed in the input view. We quantify the disparity between the color distributions using Chamfer Distance, which treats the pixels from both views as point clouds within the RGB color space.

\begin{multline}
    \mathcal{L}_\mathrm{CD}(\mathbf{F}_\mathbf{x},\mathbf{F}_\mathcal{I}) \\ = \sum_{x \in \mathbf{F}_\mathbf{x}} \operatorname*{min}_{y \in \mathbf{F}_\mathcal{I}} ||x-y||^2_2 + \sum_{y \in \mathbf{F}_\mathcal{I}} \operatorname*{min}_{x \in \mathbf{F}_\mathbf{x}} ||x-y||^2_2,
\end{multline}
where $\mathbf{F}_\mathbf{x}$ represents the foreground pixels of the novel-view albedo rendering  $\mathbf{x}$, and $\mathbf{F}_\mathcal{I}$ corresponds to the foreground pixels of the input view $\mathcal{I}$.

\qheading{Camera sampling during optimization}
%
To optimize the 3D model using multi-view renderings, cameras are randomly sampled in a way that ensures comprehensive coverage of the entire body by adjusting various parameters. The ratio $p_\mathrm{body}$ determines the sampling probability of body, while the height $h_\mathrm{body}$, radius $r_\mathrm{body}$, rotation $\theta_\mathrm{body}$, and azimuth ranges $\phi_\mathrm{body}$ are adjusted relative to the \smplx body scale. 
% 
By employing this approach, we can effectively incorporate both global and local views into the sampling process. Consequently, it facilitates the recovery of a complete representation of the body's appearance while ensuring accurate alignment of local details.

%
To mitigate the occurrence of mirrored appearance artifacts, we incorporate view-aware prompts (``front/side/back/overhead view'') according to the viewing angle. This approach has demonstrated its effectiveness in \db~\cite{poole2022dreamfusion}.
%
In order to improve facial details, we sample cameras positioned around the face, with a probability of $p_\mathrm{face} = 1-p_\mathrm{body}$ and specific parameters including height $h_\mathrm{face}$, radius $r_\mathrm{face}$, rotation $\theta_\mathrm{face}$, and azimuth $\phi_\mathrm{face}$. Additionally, for the cameras positioned around the face, we include an additional prompt ``the face of'' to enhance the textual guidance.
%

% \qheading{Overall Losses} Here we summarize the losses we use for each training iteration. First, we randomly decide whether to supervise the color renderings, surface normal renderings, or shaded rendering with chances of $p_\mathrm{color}$, $p_\mathrm{normal}$ and $p_\mathrm{shaded}$ to achieve alignment between the reconstructed geometry and the texture. For simplicity, we combine the sampling probabilities into the loss weights in the following equation to formulate our overall training loss.


\qheading{Overall Loss} 
%
The overall loss is defined as follows:
%
\begin{align}
\begin{split}
\label{overall_l}
    \mathcal{L}_\mathrm{overall} &= \lambda_\mathrm{SDS}\mathcal{L}_\mathrm{SDS} + \mathcal{L}_\mathrm{recon} + \mathcal{L}_\mathrm{reg}\\
    \mathcal{L}_\mathrm{SDS} & = p_\mathrm{color}\mathcal{L}_\mathrm{SDS}^\mathrm{color} + p_\mathrm{normal}\mathcal{L}_\mathrm{SDS}^\mathrm{normal} + p_\mathrm{shaded}\mathcal{L}_\mathrm{SDS}^\mathrm{shaded} \\ \mathcal{L}_\mathrm{recon} & = \lambda_\mathrm{recon}\mathcal{L}_\mathrm{recon} + \lambda_\mathrm{mask}\mathcal{L}_\mathrm{mask} \\
    \mathcal{L}_\mathrm{reg} & = \lambda_\mathrm{norm}\mathcal{L}_\mathrm{norm}  + \lambda_\mathrm{CD}\mathcal{L}_\mathrm{CD} +\lambda_\mathrm{lap}\mathcal{L}_\mathrm{lap} , 
\end{split}
\end{align}
%
where all the $\lambda$s are the weights to balance various losses.
%
Specifically, we randomly decide whether to supervise the color renderings, surface normal renderings, or shaded rendering with selected probability $p_\mathrm{color}$, $p_\mathrm{normal}$ and $p_\mathrm{shaded}$ to enhance the alignment between the reconstructed geometry and the texture. For more detailed information about these hyperparameters, please refer to the \supmat
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Improving for high-quality reconstruction}
\subsection{Two-stage Optimization} \label{sec:multistage}

%
For stable and robust optimization, we propose a two-stage strategy: 1) Geometry Stage: refining full-body geometry from coarse to fine; 2) Texture Stage: generating view-consistent full-body texture.
%

\qheading{I. Geometry-stage: coarse-to-fine geometry refinement}
%
As discussed in~\cref{dmtet}, to achieve high-resolution mesh reconstruction, we utilize subdivision on the \dmtet. Hence, the optimization is performed in two stages: first, w/o subdivision for $t_\mathrm{coarse}$ iterations, and then with subdivision for $t_\mathrm{fine}$ iterations. To ensure robust convergence of the geometry, we use $\mathcal{L}_\mathrm{norm}$ in~\cref{loss-normal} to regularize the geometric surface with normal estimations. Empirically, we start with a higher value of $\lambda_\mathrm{norm}$ during each stage and gradually decrease it using cyclic cosine annealing:
\begin{multline}
\lambda_\mathrm{norm} (t) =\\
\begin{cases}
0.5 \lambda_\mathrm{norm} \left(1 + \cos\left(\frac{t}{t_\mathrm{coarse}}\pi\right)\right) & \text{if } t < t_\mathrm{coarse} \\
0.5 \lambda_\mathrm{norm} \left(1 + \cos\left(\frac{t-t_\mathrm{coarse}}{t_\mathrm{fine}}\pi\right)\right) & \text{if } t \geq t_\mathrm{coarse}
\end{cases},
\end{multline}
%
where $\lambda_\mathrm{norm} (t)$ represents the weight of $\mathcal{L}_\mathrm{norm}$ at the $t$-th iteration, and $\lambda_\mathrm{norm}$ is the base setting for the loss weight. 

We adopt the ``hand replacement'' proposed in ECON~\cite{xiu2022econ} to initially register the final \dmtet output with the \smplx body model. Subsequently, we replace the hand geometries with \smplx ones. This replacement effectively mitigates any potential artifacts introduced during reposing and facilitates a smoother transition to the subsequent texture generation stage.

\qheading{II. Texture-stage: full \& consistent texture generation} 
%
In order to enhance the overall quality of the reconstructed full-body texture, we tackle issues related to self-occlusion and over-saturated colors in a secondary stage of texture refinement. This is achieved by incorporating supervision from both A-pose and input pose renderings and utilizing the Chamfer distance color consistency loss $\mathcal{L}_\mathrm{CD}$. 

In the second stage, we maintain the post-processed meshes of the input pose ($\mathcal{M}_\mathrm{In}$) and the A-pose ($\mathcal{M}_\mathrm{A}$). Both poses' albedo renderings are supervised using $\mathcal{L}_\mathrm{SDS}^\mathrm{color}$ with a weighting ratio of $p_\mathrm{pose}$. The textures of $\mathcal{M}_\mathrm{In}$ and $\mathcal{M}_\mathrm{A}$ are modeled by $\Psi_\mathrm{color}$ in the 3D space of the input pose, we optimize the texture from scratch in the second stage with $Psi_\mathrm{}$ randomly re-initialized, rather than fin-tuning based on the texture results of the first stage. Additionally, to ensure accurate alignment between texture and geometry, pixel-wise input view reconstruction of $\mathcal{M}_\mathrm{pose}$ is enforced through $\mathcal{L}_\mathrm{recon}$. To handle occluded regions, a self-occlusion mask denoted as $m_\mathrm{occ}$ is introduced, which masks $\mathcal{L}_\mathrm{recon}$ accordingly.
% 
Upon convergence of the full-body texture, an additional optimization phase is initiated, lasting for $t_\mathrm{color}$ iterations. During this phase, we utilize $\mathcal{L}_\mathrm{CD}$ to enforce color consistency.


\begin{comment}
\qheading{Stage 1: robust recovery of 3D clothed body} 
% In the previous section, we introduce the normal estimation results in $\mathcal{L}_\mathrm{normal}$ we use to regularize the front-view and back-view surfaces. This is necessary for a robust convergence of the early stage of training and produces an approximate clothed body shape and a semantically plausible texture. In this stage, we enforce the \dmtet grid offsets $\Delta v_i$ to be zero, and only train the SDF value $s(v_i)$ for robustness. The overall training loss in this stage is formulated as follows:
% \begin{equation}
% \begin{aligned}
%     \mathcal{L}_\mathrm{stage1} &= \lambda_\mathrm{SDS}\left(p_\mathrm{color}\mathcal{L}_{SDS}^\mathrm{color} + p_\mathrm{normal}\mathcal{L}_{SDS}^\mathrm{normal} + p_\mathrm{shaded}\mathcal{L}_{SDS}^\mathrm{shaded}\right) \\ &+ \lambda_\mathrm{recon}\mathcal{L}_\mathrm{recon} + \lambda_\mathrm{normal}\mathcal{L}_\mathrm{normal} + \lambda_\mathrm{lap}\mathcal{L}_\mathrm{lap} , 
% \end{aligned}
% \end{equation}
We use the overall loss \eref{overall_l} to produces an approximated clothed body shape and a semantically plausible texture, especially, by enforcing $\mathcal{L}_\mathrm{normal}$.
%

\qheading{Stage 2: creating more detailed geometry details} 
% Since the estimated normal maps are commonly over-smoothed, especially for the back-side which lacks visual cues. 
% After getting the approximate reconstruction with a smooth surface from the first stage, we remove $\mathcal{L}_\mathrm{normal}$ from the training losses in this stage, and allow the geometry network to learn the tetrahedra grid offset $\Delta v_i$ to recover detailed clothed body geometry with the text guidance in SDS losses, and we still keep $\mathcal{L}_\mathrm{lap}$ to maintain surface smoothness.
% \begin{equation}
% \begin{aligned}
%     \mathcal{L}_\mathrm{stage2} &= \lambda_\mathrm{SDS}\left(p_\mathrm{color}\mathcal{L}_{SDS}^\mathrm{color} + p_\mathrm{normal}\mathcal{L}_{SDS}^\mathrm{normal} + p_\mathrm{shaded}\mathcal{L}_{SDS}^\mathrm{shaded}\right) \\ &+ \lambda_\mathrm{recon}\mathcal{L}_\mathrm{recon} + \lambda_\mathrm{lap}\mathcal{L}_\mathrm{lap} , 
% \end{aligned}
% \end{equation}
%
The reconstructed body mesh from the first stage tends to have a smooth surface, due to the over-smooth estimated normal map, especially, on the back-side of the body.
%
Therefore, in the second stage, we remove $\mathcal{L}_\mathrm{normal}$ by setting $\lambda_{recon}=0$ in \eref{overall_l} to generate more detailed geometry details by learning the tetrahedra grid offset $\Delta v_i$.
%

\qheading{Stage 3: creating consistent texture colors} 
% After the first two-stage of training, we can get a textured mesh with detailed structure and semantically consistent detailed structure.  However, as mentioned in the previous SDS-based 3D generation methods\cite{poole2022dreamfusion, lin2022magic3d, tang2023make}, since SDS uses a large guidance scale for 3D generation ($w = 100$), which is significantly large than the guidance scale used in T2I $w\in[5,30]$, the texture color generated by SDS is often over-saturated. We also find a large $w$ will overemphasize the patterns on the clothes.
% Both problems lead to unrealistic textures. To address this issue, to recover consistent colors for the occluded appearance, we also added a third stage of the training to refine the texture color. 
% In the third stage, we freeze the geometry network $\psi_\mathrm{g}$ and only fine-tune the color network $\psi_\mathrm{c}$ with a smaller $w_\mathrm{refine}=10$ which is approximate to the guidance scale used in T2I generation and only use albedo rendering in the training process to further refine the texture color.
%
In the third stage, we freeze the geometry network $\psi_\mathrm{g}$ and fine-tune the color network $\psi_\mathrm{c}$ by only using the albedo rendering in the training process to further refine the texture color.
%
%\begin{equation} \label{stage3}
%    \mathcal{L}_\mathrm{stage3} = \lambda_\mathrm{SDS}\mathcal{L}_{SDS}^\mathrm{color} + \lambda_\mathrm{recon}\mathcal{L}_\mathrm{recon} . 
%\end{equation}
%
In contrast to previous SDS-based 3D generation methods \cite{poole2022dreamfusion, lin2022magic3d, tang2023make} with large guidance scale $w\in[5,30]$, which tend to generate over saturated colors and overemphasized cloth patterns, we use a smaller $w_\mathrm{refine}=10$ which is similar to the guidance scale used in the T2I generation.
%    
\end{comment}



\begin{comment}
\subsubsection{Edge-conditioned SDS for detailed geometry alignment}

Recent progress in controllable T2I diffusion models \cite{zhang2023adding} enables users to use extra image conditions to control the layout of the generated images, such as edge maps, pose annotations, depth maps, etc. Here we also employ one of the pre-trained ControlNet modules from \cite{zhang2023adding} in $\mathcal{L}_\mathrm{SDS}^g$ to improve the consistency of geometry details and texture details. For the current training view $\mathrm{k}$, we first render $x\mathrm{ref}=\mathcal{C}(\psi_\mathrm{g}$ as a reference image to guide the generation of geometry details. We extract the Canny edge map of the reference image as the condition of the layout $\textbf{l}^x_\mathrm{ref}$ in $\mathcal{L}_\mathrm{SDS}^g$.

\begin{equation}
    \nabla_{\psi_\mathrm{g}}\mathcal{L}_\mathrm{SDS}^\mathrm{g}(\mathbf{k}, \mathbf{n}, \mathbf{c}^{P_\mathrm{g}}, \textbf{l}^x_\mathrm{ref})= \mathbb{E}_{\mathrm{t, \epsilon}}\left[ w_t \left(\hat{\epsilon}_{\phi'}(\mathbf{z}_t^\mathbf{n};\mathbf{c}^{P_\mathrm{g}},\textbf{l}^x_\mathrm{ref},t)-\epsilon\right)\frac{\partial \mathbf{n}}{\partial \psi_\mathrm{g}}\frac{\partial z^\mathbf{n}}{\mathbf{n}}\right], 
\end{equation}

We only back-propagate the gradient to $\psi_\mathrm{g}$ here to update the geometry.    
\end{comment}


==> tabtex/summary.tex <==
\definecolor{Gray}{gray}{0.92}

\begin{table}[]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccccc}
Methods        & Input data  & Training data     & \begin{tabular}{c}Body motion
  \end{tabular}      & \begin{tabular}{c}Face motion
  \end{tabular}     & \begin{tabular}{c}Textured meshes
  \end{tabular}    \\ \hline
\begin{tabular}[c]{@{}c@{}}AvatarCraft\cite{jiang2023avatarcraft}\end{tabular} & \multirow{1}{*}{Text}      
& \multirow{1}{*}{Data-free} & \xmark & \xmark & \xmark \\
\hline
DreamAvatar\cite{cao2023dreamavatar}    & Text & \multirow{1}{*}{Data-free} & \cmark & \xmark & \xmark \\
\hline
\begin{tabular}[c]{@{}c@{}}PHORHUM\cite{alldieck2022photorealistic}\end{tabular}    & \multirow{1}{*}{Image}      & \begin{tabular}{c}3d scans
  \end{tabular}             & \cmark & \xmark & \cmark \\
\hline
\begin{tabular}[c]{@{}c@{}}SHERF\cite{hu2023sherf}\end{tabular} & Image & \begin{tabular}{c}Multi-view
  \end{tabular} & \cmark & \xmark & \xmark \\
\hline

EVA3D \cite{hongEVA3DCompositional3D2022}         & Latent code & \begin{tabular}{c}Posed images
  \end{tabular}   & \cmark & \xmark & \xmark \\
\hline

Rodin  \cite{wang2022rodin}                 & \multirow{1}{*}{Text \& Image} & \begin{tabular}{c}3D synthesis
  \end{tabular}        & \xmark & \cmark & \xmark \\
\hline
\rowcolor{Gray} 
Ours           & \multirow{1}{*}{Text \& Image} & Data-free         & \cmark & \cmark & \cmark \\ 
\end{tabular}}
\caption{\footnotesize\label{table:methodComparison} \textbf{Recent avatar creation methods that are most relevant to our work.} Ours is the first work that 1) supports a single image or text description as input. 2) does not require human-specific training data. 3) supports expressive animation with the body, the face, and the hands. 4) can generate high-resolution textured meshes of the character. (\TODO{MODIFY THIS TABLE! make sure it is referenced in the text})}
\end{table}
